Learning multiview 3D point cloud registration

We present a novel, end-to-end learnable, multiview 3D point cloud registration algorithm. Registration of multiple scans typically follows a two-stage pipeline: the initial pairwise alignment and the globally consistent refinement. The former is often ambiguous due to the low overlap of neighboring point clouds, symmetries and repetitive scene parts. Therefore, the latter global refinement aims at establishing the cyclic consistency across multiple scans and helps in resolving the ambiguous cases. In this paper we propose, to the best of our knowledge, the first end-to-end algorithm for joint learning of both parts of this two-stage problem. Experimental evaluation on well accepted benchmark datasets shows that our approach outperforms the state-of-the-art by a significant margin, while being end-to-end trainable and computationally less costly. Moreover, we present detailed analysis and an ablation study that validate the novel components of our approach. The source code and pretrained models are publicly available under https://github.com/zgojcic/3D_multiview_reg.

==> sections/algorithm.tex <==
\begin{algorithm}[t!]
\caption{Pseudo-code of the proposed approach}\label{alg:3d_mul_reg}
    \small{\begin{algorithmic}
    
        \State{Input: a set of potentially overlapping scans $\{\mathbf{S}_i\}_{i=1}^{N_{\mathcal{S}}}$}
        \State{Output: globally optimized poses $\{\mathbf{M}_i^{*}\}_{i=1}^{N_{\mathcal{S}}}$}
        \State{\textcolor{bostonuniversityred}{\textit{\# Compute the pairwise transformations}}}\\
        \For{each pair of scans $\mathbf{S}_i, \mathbf{S}_j \subset \mathcal{S}, i \neq j$}{
        \State{\text{- }$\mathbf{X}_{ij}=\operatorname{cat}([\mathbf{S}_i, \phi(\mathbf{S}_i,\mathbf{S}_j)])\in\mathbb{R}^{N_{\mathbf{S}_i}\times 6}$}
        \State {\text{- }$\mathbf{w}_{ij}=\psi_{init}(\mathbf{X}_{ij})\in\mathbb{R}^{N_{\mathbf{S}_i}}$}
        \State{\text{- }calculate $\mathbf{R}_{ij}, \mathbf{t}_{ij}$ using SVD according to \eqref{eq:weighted_pairwise}}
        }
        \State{\textcolor{bostonuniversityred}{\textit{\# Iterative network for transformation synchronization}}}
        \State{$\mathbf{X}_{ij}^{(0)}\leftarrow \mathbf{X}_{ij}$, $\mathbf{w}_{ij}^{(0)}\leftarrow \mathbf{w}_{ij}$, $\mathbf{r}_{ij}^{(0)}\leftarrow \mathbf{r}_{ij}$}\\
        \For{$k=1,2,\cdots,\mathrm{max\_iters}$}{
            \hspace{-2ex}\For{each pairwise output from $\psi_{init}$}{
                \State{\text{- }$\mathbf{R}_{ij}^{(k)}, \mathbf{t}_{ij}^{(k)}, \mathbf{w}_{ij}^{(k)}=\psi_{iter}([\mathbf{X}_{ij}^{(k-1)}, \mathbf{w}_{ij}^{(k-1)}, \mathbf{r}_{ij}^{(k-1)}])$}
                \State{\text{- }estimate $\textit{local}\{c^{(k)}_{ij}\}$ using \eqref{eq:local_conf}}
            }
            \State{\text{- }Gather the pairwise estimation as $\mathbf{R}^{(k)}, \mathbf{t}^{(k)}, \mathbf{c}^{(k)}$}\\ %
            \If{$k=1$}{
                \hspace{-4ex}\text{- }$\mathbf{c}^{(k)}:= \textit{local}\{\mathbf{c}^{(k)}\}$
            }
            \hspace{-4ex}\Else
            {
                \hspace{-4ex}\text{- }$\mathbf{c}^{(k)}:= {f}_{HM}(\textit{local}\{\mathbf{c}^{(k)}\} , \textit{global}\{\mathbf{c}^{(k-1)}\}$
            }
            \State{\text{- }$\mathbf{R}^{*(k)}, \mathbf{t}^{*(k)} = \operatorname{Transf\text{-}Sync}(\mathbf{R}^{(k)}, \mathbf{t}^{(k)},\mathbf{c}^{(k)})$}\\
            \For{each pair of scans $\mathbf{S}_i, \mathbf{S}_j \subset \mathcal{S}, i \neq j$}{
                \State{\text{- }$\mathbf{X}_{ij}^{(k+1)}=\operatorname{cat}([\mathbf{S}_i, \mathbf{M}_{ij}^{*(k)}\otimes\phi(\mathbf{S}_i,\mathbf{S}_j)]$}
                \State{\text{- }$\mathbf{w}_{ij}^{(k+1)}=\mathbf{w}_{ij}^{(k)}$}
                \State{\text{- }$\mathbf{r}_{ij}^{(k+1)}=\|\mathbf{S}_i - \mathbf{M}_{ij}^{*(k)}\otimes\phi(\mathbf{S}_i,\mathbf{S}_j)\|_{2}$}
            }
            }
    \end{algorithmic}}
\end{algorithm}

==> sections/section-trans-sync.tex <==
\section{General Idea}

Let $\mathbf{p}_i = [x_i,y_i,z_i]$ refer to the 3D coordinates of a point and $\mathbf{P} \in \mathbb{R}^{N \times 3}$ to a collection of such points also denoted as a point cloud. In our notation $(\mathbf{P})_i$ refers to the $i$-th row of the matrix $\mathbf{P}$ such that $(\mathbf{P})_i = \mathbf{p}_i$. Consider a set of $n$ potentially overlapping point clouds $\mathcal{P} = \{\mathbf{P}_i, 1 \leq i \leq n \}$. Our task is to find a globally optimal solution that aligns these $n$ point clouds in a common reference frame.
From $n$ point clouds we can form $\binom{n}{2}$ point cloud pairs that might or might not overlap. Let $\{ \mathbf{P}, \mathbf{Q} \}$ represent one of those point cloud pairs such that $\mathbf{P} := \mathbf{P}_i$ and $\mathbf{Q} := \mathbf{P}_j$. If $\mathbf{P}$ and $\mathbf{Q}$ do overlap there exist a bijective function that maps the points of $\mathbf{P}$ to their corresponding points in $\mathbf{Q}$. Assuming a static scene and rigid point clouds, this relation is described by the parameters of the congruent transformation
\begin{equation}
    \mathbf{Q} = \mathbf{K}\mathbf{P}\mathbf{R}_{ij}^{T}  + \mathbf{1}\otimes\mathbf{t}_{ij}^{T}
\end{equation}
where $\mathbf{K} \in \mathbb{P}^{|\mathbf{P}'_j|}$ is a permutation matrix whose eneteries $k_{ij} = 1$ if $(\mathbf{P})_i$ corresponds to $(\mathbf{Q})_j$ and 0 otherwise. $\mathbf{R}_{ij} \in SO(3)$ and $\mathbf{t} \in \mathbb(R)^3$ are the relative transformation matrix and translation vector that orient point cloud $\mathbf{P}$ to point cloud $\mathbf{Q}$, respectively. The relative pose $\mathbf{T}_{ij} \in SE(3)$ can then be expressed as
\begin{equation}
    \mathbf{T}_{ij} = \begin{bmatrix} 
\mathbf{R}_{ij} & \mathbf{t}_{ij} \\
\mathbf{0}^T & 1 
\end{bmatrix}
\end{equation}
If the permutation matrix $\mathbf{K}$ the optimal $\mathbf{R}^*_{ij}$ and $\mathbf{t}^*_{ij}$, in the weighted least squares sense, are the solution to
\begin{equation}
    (\mathbf{R}^*_{ij},\mathbf{t}^*_{ij}) = \operatorname*{argmin}_{\mathbf{R}_{ij},\mathbf{t}_{ij}} \sum_{k=1}^n w_k ||(\mathbf{R}_{ij}\mathbf{p}_k^T  + \mathbf{t}_{ij})^T - \mathbf{q}_k ||^2  
\label{eq:least_squares}
\end{equation}
where Eq. \ref{eq:least_squares} admits a closed-form solution which is differentiable (see Sec.~\ref{sec:closed_form_ls}). 

\subsection{Weighting network}
Eq.~\ref{eq:least_squares} holds under the assumption that each point $\mathbf{q}_k$ is the actual correspondence of the point $\mathbf{p}_k$, which is equivalent to the assumping an error free permutation matrix $\mathbf{K}_{ij}$. We determine the matrix $\mathbf{K}_{ij}$ using the correspondence search in the feature space. More specifically, we randomly sample $n_f := 5000$ interest points from each point cloud and we infer their 32- dim local feature descriptors using 3DSmoothNet~\cite{gojcic20193DSmoothNet}. The putative correspondences are then established using the nearest neighbor search in the feature space. Naturally, these putative correspondences are very noisy and contain outliers. In this case Eq.~\ref{eq:least_squares} will yield wrong estimates unless the weights $w_k$ are set to zero for all outliers. However, the outliers are not known beforehand and cannot be trivially identified. We therefore follow the idea of~\cite{ranftl2018deepFundamentalMatrix} and learn the weights from the data. 
Our deep network, used to represent the complex learned weighting function, is adopted from~\cite{zhang2019oanet}. It maps the input $\mathbf{X} \in \mathbb{R}^{N \times 6}$ to a vector of weights $\mathbf{w} \in \mathbb{R}^N$ where $w_k \in [0,1]$. The input $\mathbf{X}$ contains solely the coordinates of the putative correspondences $\mathbf{c_k} = [x_k,y_k,z_k,x_k,y_k,z_k]$ where 
\begin{equation}
    \mathbf{X} = [c_{1};\ldots; c_{n_{f}}] 
\end{equation}
The network architecture is based on the PointNet architecture in order to ensure the equivariance of the network to input perturbation. The global information is aggregated using two Instance normalization layers in each of the ResNet layer blocks. Additionally, after 3 ResNet blocks the DiffPool layer maps the unordered nodes to a set of ordered clusters, which are used to exploit the local context. 



\begin{figure*}[!ht]
	\begin{center}
		\includegraphics[width=0.95\linewidth]{./figures/Network_Filtering.png}
	\end{center}
	\vspace{-1ex}
	\caption{\textbf{OANet filtering network architecture:} Building blocks of the OANet filtering network without the confidence level estimation. Some parts of the figure are taken from \url{https://arxiv.org/pdf/1908.04964.pdf}. All the perceptron layers (green squares) share the weights across the correspondences. After the first 3 ResNet layers the unordered points are assigned via a soft assignment to $M=500$ clusters. In the bottom layer of the network 3x OA. }
	\label{fig:network_architecture}
\end{figure*}

\section{Closed-form solution for Eq. \ref{eq:least_squares}}
\label{sec:closed_form_ls}
Let $\overline{\mathbf{p}}$ and $\overline{\mathbf{q}}$ 
\begin{equation}
    \overline{\mathbf{p}} = \frac{\sum^n_{k=1} w_i \mathbf{p}_i}{\sum^n_{k=1} w_i}, \quad
    \overline{\mathbf{q}} = \frac{\sum^n_{k=1} w_i \mathbf{q}_i}{\sum^n_{k=1} w_i}
\end{equation}
denote weighted centroids of point clouds $\mathbf{P}$ and $\mathbf{Q}$ respectively. We can then compute the centered point coordinates as 
\begin{equation}
    \mathbf{p}'_k := \mathbf{p}_k - \mathbf{\overline{\mathbf{p}}}, \quad \mathbf{q}'_k := \mathbf{q}_k - \mathbf{\overline{\mathbf{q}}}, \quad k = 1,\ldots, n
\end{equation}
Arranging the centered point back to the matrix form, a weighted covariance matrix $\mathbf{S} \in \mathbb{R}^{3 \times 3}$ can be computed as 
\begin{equation}
    \mathbf{S} = \mathbf{P}'\mathbf{W}\mathbf{Q}'^T
\end{equation}
where $\mathbf{W} = diag(w_1,\ldots,w_n)$ . Considering the singular value decomposition $\mathbf{S}=\mathbf{U}\mathbf{\Sigma}\mathbf{V}^T$ the solution to Eq.~\ref{eq:least_squares} is given by
\begin{equation}
    \mathbf{R}^*_{ij} = \mathbf{V}\mathbf{I}\mathbf{U}^T  
\end{equation}
where $\mathbf{I} \in \mathbb{R}^{3 \times 3}$ is an identity matrix with the bottom-most element multiplied by $det(\mathbf{V}\mathbf{U}^T)$ to avoid creating a reflection matrix. Finally, $\mathbf{t}^*_{ij}$ is computed as
\begin{equation}
    \mathbf{t}^*_{ij} = \overline{\mathbf{q}} - (\mathbf{R}^*_{ij}\overline{\mathbf{p}}^T)^T
\end{equation}

 



\begin{table*}[!t]
	\centering
	\resizebox{0.9\textwidth}{!}{\begin{tabular}{l|cccccccccccccc}
			\hline
			&FPFH~\cite{rusu2009FPFH}&3DMatch~\cite{zeng20163dmatch}&CGF~\cite{khoury2017CGF}&PPFNet~\cite{deng2018ppfnet}&FCGF& 3DSN &3DSN(m) + Filt. &FCGF + Filt. &FCGF(m) + Filt. \\
			\hline\hline
            Kitchen&$0.36$&$0.85$&$0.72$&$0.90$&$0.93$&$0.96$&$0.93$&$0.95$&$0.97$\\
            Home 1 &$0.56$&$0.78$&$0.69$&$0.58$&$0.91$&$0.88$&$0.85$&$0.95$&$0.95$\\
            Home 2 &$0.43$&$0.61$&$0.46$&$0.57$&$0.71$&$0.79$&$0.72$&$0.71$&$0.75$\\
            Hotel 1&$0.29$&$0.79$&$0.55$&$0.75$&$0.91$&$0.95$&$0.92$&$0.93$&$0.94$\\
            Hotel 2&$0.36$&$0.59$&$0.49$&$0.68$&$0.87$&$0.83$&$0.81$&$0.90$&$0.91$\\
            Hotel 3&$0.61$&$0.58$&$0.65$&$0.88$&$0.69$&$0.92$&$0.89$&$0.85$&$0.85$\\
            Study  &$0.31$&$0.63$&$0.48$&$0.68$&$0.75$&$0.84$&$0.80$&$0.81$&$0.88$\\
            MIT Lab&$0.31$&$0.51$&$0.42$&$0.62$&$0.80$&$0.76$&$0.76$&$0.80$&$0.80$\\
			\hline
			Average&$0.40$&$0.67$&$0.56$&$0.71$&$0.82$&$0.86$&$0.83$&$0.86$&$0.88$\\
			\hline
	\end{tabular}}
	\caption{\textbf{Detailed quantitative results on the \textit{3DMatch} dataset.} For each scene we report the average recall in percent over all overlapping fragment pairs. Best performance is shown in bold.}
	\label{tab:results_3DMatch_dataset}
\end{table*}


\begin{figure}[!ht]
	\begin{center}
		\includegraphics[width=0.95\linewidth]{./figures/Confidence_EST.PNG}
	\end{center}
	\vspace{-1ex}
	\caption{\textbf{Confidence estimation}}
	\label{fig:network_architecture}
\end{figure}

\section{Intermediate results of transformation synchronization}
This section includes a short introduction to the transformation synchronization module and presents the intermediate results of performing synchronization on different set of scans, which have different connectivity (i.e. the overlap between each pair of scans)

\subsection{Relation to the proposal}
The transformation synchronization (tran-sync in short) is carried for globally refining the pairwise transformations of multi-scans estimated by the filtering network. The trans-sync module consists of two parts: spectral decomposition and graph update. The former is based on the spectral analysis, which is applied to compute the global transformation matrix using the Laplacian of the graph consisting of the multi-scans. The latter is a scheme generator, which computes the policy of updating the graph by combining the global transformation residuals and the confidence level of pairwise transformation estimation. 

\todo{Add the description of spectral decomposition}: spectral analysis -- differentiable

\todo{Add the reweighting part}: iterative network -- confidence update; residuals -- IRLS; joint reweighting scheme (e.g., $\beta$-F score)

\todo{Add the sub-network for synchronization}


\subsection{Results}
The spectral decomposition and graph udpate scheme are implemented according to \todo{CITE}\footnote{Huang et al. 2019, Learning Transformation Synchronization.} and \todo{CITE} \footnote{Arrigoni et al. 2015, Spectral Motion Synchronization in SE(3).}, respectively. The input to the tran-sync module consists of the relative transformation estimation from the filtering network. The angular and translation errors are computed as the same in \todo{CITE}. Two scenes (Kitchen and MIT-Lab) from 3DMatch dataset has been taken as the examples to illustrate the impact of graph connectivity on the performance of tran-sync. The connectivity between the fragments are visualized in Fig.\ref{fig:scan_con_graph}.

\begin{figure}
    \centering
    \subfloat[Kitchen]{\includegraphics[width=0.85\linewidth]{./figures/scan_graph_kitchen.pdf}
    \label{subfig:con_graph_kit}}\\
    \subfloat[MIT-Lab. The two sub-graphs are named as sub-1 (the left one) and sub-2 (the right one).]{\includegraphics[width=0.85\linewidth]{./figures/scan_graph_erika.pdf}
    \label{subfig_con_graph_mit}}
    
    \caption{The connectivity graph of scene kitchen and MIT-Lab}
    \label{fig:scan_con_graph}
\end{figure}

\subsection{Tran-sync on kitchen}
As shown in Fig.\ref{subfig:con_graph_kit}, the fragments of scene kitchen are well overlapped and form quite a number of cycles. In this case, it is helpful for the global tran-sync. This is also validated by the large reduction of angular and translation errors (Fig.\ref{fig:cmp_ae_te_full_kit})after tran-sync comparing to the ones before tran-sync.
\begin{figure}
    \centering
    \subfloat[Angular error (AE)]{\includegraphics[width=0.85\linewidth]{./figures/cmp_ae_full_graph_kitchen.pdf}}\\
    \subfloat[Translation error (TE)]{\includegraphics[width=0.85\linewidth]{./figures/cmp_te_full_graph_kitchen.pdf}}
    
    \caption{Comparison of tran-sync performance on kitchen}
    \label{fig:cmp_ae_te_full_kit}
\end{figure}

\subsection{Tran-sync on MIT-Lab}
When treating the scene MIT-lab as one graph, the tran-sync fails to work. This is due to the disconnectivity between the fragments as shown in Fig.\ref{subfig_con_graph_mit}. The framgents form four disconnect sub-graphs. In this case, the spectral decomposition does not work well because the estimation eigen-vectors, the key to estimating the global rotations, of the Laplacian does not well properly. 
\begin{figure}
    \centering
    \subfloat[Angular error (AE)]{\includegraphics[width=0.85\linewidth]{./figures/cmp_ae_full_graph_erika.pdf}}\\
    \subfloat[Translation error (TE)]{\includegraphics[width=0.85\linewidth]{./figures/cmp_te_full_graph_erika.pdf}}
    
    \caption{Comparison of tran-sync performance on MIT-Lab treating the whole scene as one graph}
    \label{fig:cmp_ae_te_full_mit}
\end{figure}

We have also tested the scenario of taking the two sub-graph as the independent one for tran-sync. The results on these two sub-graphs show that the tran-sync approach can refine the global registration when the fragments consist of one graph. This point also suggests that it would be a bit tricky if the edges are removed adaptively during the optimization step. Because the connectivity of the graph might be changed in the way of crashing the tran-sync approach.

In addition, we can see from Fig.\ref{fig:cmp_ae_te_sub_1_mit} and \ref{fig:cmp_ae_te_sub_2_mit} that the level of connectivity (may quantified as cycles) between the fragments has an impact on the global refinement of the transformation estimation. The graph sub-1 has fewer number cycles than graph sub-2. In this case it results in less reduction of transformation errors as comparing graph sub-1 to sub-2 as shown in Fig.\ref{fig:cmp_ae_te_sub_1_mit} and \ref{fig:cmp_ae_te_sub_2_mit}.

\begin{figure}
    \centering
    \subfloat[Angular error (AE)]{\includegraphics[width=0.85\linewidth]{./figures/cmp_ae_sub_1_graph_erika.pdf}}\\
    \subfloat[Translation error (TE)]{\includegraphics[width=0.85\linewidth]{./figures/cmp_te_sub_1_graph_erika.pdf}}
    
    \caption{Comparison of tran-sync performance on MIT-Lab of sub-1}
    \label{fig:cmp_ae_te_sub_1_mit}
\end{figure}

\begin{figure}
    \centering
    \subfloat[Angular error (AE)]{\includegraphics[width=0.85\linewidth]{./figures/cmp_ae_sub_2_graph_erika.pdf}}\\
    \subfloat[Translation error (TE)]{\includegraphics[width=0.85\linewidth]{./figures/cmp_te_sub_2_graph_erika.pdf}}
    
    \caption{Comparison of tran-sync performance on MIT-Lab  of sub-2}
    \label{fig:cmp_ae_te_sub_2_mit}
\end{figure}

\subsection{Comparison of the tran-sync performance}
Fig.\ref{fig:cmp_trans_error_ran_fil_conf_iter_1_kit} and Fig.\ref{fig:cmp_trans_error_ran_fil_conf_kit} presents the comparison of the tran-sync performance using different estimation as the input. It shows that with the help of tran-sync the filtering estimation can be largely refined and is caple of achieving on par accuracy as using the RANSAC estimation as the input. Though the RANSAC estimation is better than that of the filtering one before carring out the tran-sync.

\begin{figure}
    \centering
    
    \subfloat[AE]{\includegraphics[width=0.85\linewidth]{figures/cmp_ae_ran_fil_conf_iter_1.pdf}
    \label{subfig:cmp_ae_ran_fil_conf}}\\
    \subfloat[TE]{\includegraphics[width=0.85\linewidth]{figures/cmp_te_ran_fil_conf_iter_1.pdf}
    \label{subfig:cmp_te_ran_fil_conf}}
    \caption{Comparison of tran-sync using RANSAC and filtering as input with one iteration}
    \label{fig:cmp_trans_error_ran_fil_conf_iter_1_kit}
\end{figure}

\begin{figure}
    \centering
    
    \subfloat[AE]{\includegraphics[width=0.85\linewidth]{figures/cmp_ae_ran_fil_conf.pdf}
    \label{subfig:cmp_ae_ran_fil_conf}}\\
    \subfloat[TE]{\includegraphics[width=0.85\linewidth]{figures/cmp_te_ran_fil_conf.pdf}
    \label{subfig:cmp_te_ran_fil_conf}}
    \caption{Comparison of tran-sync using RANSAC and filtering as input}
    \label{fig:cmp_trans_error_ran_fil_conf_kit}
\end{figure}

\newpage
\begin{figure*}
    \includegraphics[angle=-90,origin=c,width=\linewidth,clip]{figures/Network_structure.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}

